One-Shot Doc Snippet Detection: Powering Search in Document Beyond Text

Active consumption of digital documents has yielded scope for research in various applications, including search. Traditionally, searching within a document has been cast as a text matching problem ignoring the rich layout and visual cues commonly present in structured documents, forms, etc. To that end, we ask a mostly unexplored question: "Can we search for other similar snippets present in a target document page given a single query instance of a document snippet?". We propose MONOMER to solve this as a one-shot snippet detection task. MONOMER fuses context from visual, textual, and spatial modalities of snippets and documents to find query snippet in target documents. We conduct extensive ablations and experiments showing MONOMER outperforms several baselines from one-shot object detection (BHRL), template matching, and document understanding (LayoutLMv3). Due to the scarcity of relevant data for the task at hand, we train MONOMER on programmatically generated data having many visually similar query snippets and target document pairs from two datasets - Flamingo Forms and PubLayNet. We also do a human study to validate the generated data.

==> architectural_details.tex <==
\section{Appendix}

\subsection{Additional Architectural Details}
\label{appendix:add_architecture}
\textbf{Feature Extractor.}
The image encoder is a DiT-backbone with encoder-only architecture having 4 layers, each containing 4 attention heads with model dimension of 512. The encoder takes 3 channel document image resized to 224$\times$224 resolution which is further cut into 16$\times$16 sized patches and outputs a token sequence of length 197 (CLS + (224$\times$224)/(16$\times$16)). 

As for the text encoder, we use a BeRT-based sentence transformer \cite{song2020mpnet} that generates 768 dimensional embedding for a given block of text. The continuous blocks of text in the document are fed into the encoder to generate token sequence of dimension (\# text blocks, 768). Unlike all the other MONOMER parameters, the text encoder weights are \emph{frozen}.

We implement the layout encoder using encoder-only transformer architecture with 6 layers, 8 heads and model dimension of 1024. It takes bounds of the document entities and outputs sequence of (\# bounds, 1024). Weights of this encoder are initialized randomly. All the three encoding sequences - visual, textual and spatial are further padded to maximum length of 1024.

% Third encoder used for bounding boxes is based on .... We use pretrained weights that are  finetuned to produce bounds for similar snippets while training \textit{\methodname} end-to-end. Layout transformer outputs token sequence of size (number of bounds, ). All the three sequences - visual, textual and spatial, are padded to maximum length of 1024.

\textbf{Symmetric Attention Module.}
% We use symmetric attention operation extensively to process the extracted features.
% The symmetric attention module \ref{fig:symmetric_attention}, as mentioned previously, performs multi-head attention on two sequences in symmetric manner.
The symmetric attention module consists of 2 multi-head attention (MHA) modules each containing 4 heads and embedding dimension of 512. To ensure that the input token feature dimension matches with MHA's specifications, the input sequences are passed through fully-connected layers to project feature dimension onto dimension of 512. The outputs of the MHA blocks are concatenated to obtain final token sequence with feature dimension of 1024 (512+512). 

% The outputs from the feature extractor are passed to Co-Attention module and Cross-Attention module which use symmetric attention module.
\textbf{Co-Attention and Cross-Attention Modules.}
Co-Attention Module \ref{fig:full_architecture} contains 3 symmetric attention modules one for each modality, outputting sequences $VV$, $TT$ and $SS$ of length 1024 and token size 1024. Similarly, the Cross-Attention Module \ref{fig:full_architecture} consists of 2 symmetric attention modules for generating spatio-visual features and 2 for attending text over those generated features. It generates $S_q V_t T_t$ and $S_t V_q T_q$ the dimensions of which are, once again, length of 1024 and token size of 1024. Finally we concatenate the outputs of Co-Attention and Cross-Attention blocks to create feature volume $F_{sim}$ (dimension - 1024$\times$1024$\times$5).

\textbf{Detection Head.}
The $F_{sim}$ is passed through a sequence of 5 linear layers to produce features which are reshaped to give outputs at 5 different resolutions - (1024, 8, 8, 2048), (1024, 16, 16, 1024), (1024, 32, 32, 512), (1024, 64, 64, 256), (1024, 128, 128, 128). Then we apply a standard FPN \cite{lin2017feature} to obtain features at a common representation size of $1024$. Finally, we generate proposals through an RPN \cite{girshick2014rich} and subsequently detect bounding boxes of similar crops using RoI Heads.

% $F_{sim}$ is passed through a sequence of 5 linear layers with LeakyRelu non-linearity, a dropout of $0.20$ and BatchNorm Layers. These 5 output volumes are then reshaped to features at different resolutions - (1024, 8, 8, 2048), (1024, 16, 16, 1024), (1024, 32, 32, 512), (1024, 64, 64, 256), (1024, 128, 128, 128). We use a standard FPN [CITE faster RCNN] to obtain features at a common representation size of $1024$. Finally, we generate proposals through an RPN [CITE] and subsequently detect bounding boxes using Roi Heads [CITE].

% The neck for \textit{\methodname} contains Co-Attention and Cross-Attention blocks which essentially have the same architecture [Reference to a figure]. Each block is made of $2$ multi-head attention units each comprising of $4$ heads and a matrix (or 2 matrices in case of cross-attention) to convert the input sequence tokens to the size of $512$. The block takes as input two sequences of length $1024$, performs 2 attentions - sequence 1 as query, sequence 2 as key \& value and sequence 2 as query, sequence 1 as key \& value, and concatenates the attention outputs to generate a sequence of size (1024, 512, 2). \textit{\methodname} contains 3 Co-Attention blocks - visual, textual and spatial and 4 Cross-Attention blocks - 2 for spatial-visual cross-attention and 2 for textual-spatiovisual cross-attention. As shown in figure [reference to figure/subfigure],the query and target features from the backbone are processed by the neck to produce five sequences each of size (1024, 512, 2). Further, we combine these sequences to get $(1024, 512\times5\times2)$ sized volume $F_{sim}$ which will be fed to the FPN and Detection Head.

